BARQ: A Vectorized SPARQL Query Execution Engine

Stardog is a commercial Knowledge Graph platform built on top of an RDF graph database whose primary means of communication is a standardized graph query language called SPARQL. This paper describes our journey of developing a more performant query execution layer and plugging it into Stardog's query engine. The new executor, called BARQ, is based on the known principle of processing batches of tuples at a time in most critical query operators, particularly joins. In addition to presenting BARQ, the paper describes the challenges of integrating it into a mature, tightly integrated system based on the classical tuple-at-a-time Volcano model. It offers a gradual approach to overcoming the challenges that small- to medium-size engineering teams typically face. Finally, the paper presents experimental results showing that BARQ makes Stardog substantially faster on CPU-bound queries without sacrificing performance on disk-bound and OLTP-style queries.

==> adaptive_batch_size_example.tex <==
\begin{lstfloat}[t]
\begin{lstlisting}[
%aboveskip=\smallskipamount,
%belowskip=\smallskipamount,
%float=b,
basicstyle=\ttfamily\tiny,
%language=SPARQL, 
mathescape=true,
morekeywords={Scan,NaryJoin}, 
commentstyle=\color{gray},
sensitive=true,
firstnumber=0, 
%numbers=left,
numbersep=5pt,
numberstyle=\scriptsize,
frame=none,
caption = {Adaptive Batch Size Example}, 
label={lst:adaptive_batch_size},
escapeinside={<@}{@>},
columns=flexible,
%xleftmargin=.07\textwidth, 
numberfirstline=false
]
# Legacy row-based evaluation
MergeJoin(?product), results: 2.3M
+- Scan(?product, rdf:type, :ProductType22), results: 5.7K (skip: 3)
+- Scan(?product, :producer, ?producer), results: 11K (skip: 5.5K)
+- Scan(?product, :productFeature, ?feature), <@\textcolor{sd_mediumblue}{\textbf{results: 119K}}@> (skip: 5.5K)
`- Scan(?offer, :product, ?product), results: 120K (skip: 5.5K)

# BARQ, fixed batch size for each scan operator
MergeJoin(?product), results: 2.3M (next: 4.5K), wall time: (4.5%)
+- Scan(?product, rdf:type, :ProductType22), results: 5.7K (next: 13), batched
+- Scan(?product, :producer, ?producer), results: 260K (next: 509, skip: 502), batched
+- Scan(?product, :productFeature, ?feature), <@\textcolor{sd_mediumblue}{\textbf{results: 2.0M}}@>  (next: 3.8K, skip: 3.7K), batched
`- Scan(?offer, :product, ?product), results: 1.9M (next: 3.7K, skip: 3.6K), batched

# BARQ, adaptive batch size
MergeJoin(?product), results: 2.3M (next: 4.5K), batched
+- Scan(?product, rdf:type, :ProductType22), results: 5.7K (next: 58), batched
+- Scan(?product, :producer, ?producer), results: 40K (next: 5.1K, skip: 5.0K), batched
+- Scan(?product, :productFeature, ?feature), <@\textcolor{sd_mediumblue}{\textbf{results: 139K}}@> (next: 17K, skip: 5.5K), batched
`- Scan(?offer, :product, ?product), results: 146K (next: 17K, skip: 5.5K), batched
\end{lstlisting}
\end{lstfloat}

==> lsqb_figure.tex <==
\captionsetup*[subfigure]{position=bottom,textfont=normalfont,labelfont=normalfont}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/sigmod25_barplot_lsqb_split.pdf}
    \vspace{-0.7\baselineskip}
    \caption{Mean query execution times [ms] for the LSQB benchmark.}
    \label{fig:lsqb_results}
\end{figure}

==> lsqb_query6.tex <==
\begin{lstlisting}[
%aboveskip=\smallskipamount,
%belowskip=\smallskipamount,
%float=b,
basicstyle=\ttfamily\footnotesize,
language=SPARQL, 
mathescape=true,
morekeywords={GROUP,MAX,COUNT}, commentstyle=\color{gray},
sensitive=true,
firstnumber=0, 
%numbers=left,
numbersep=5pt,
numberstyle=\scriptsize,
frame=none,
caption = {LSQB Query 6}, 
label={lst:lsqb_query6},
escapechar=",
columns=flexible,
%xleftmargin=.07\textwidth, 
numberfirstline=false
]
SELECT (COUNT(*) as ?count)
WHERE { 
 ?p1 (lp:Person_knows_Person |^lp:Person_knows_Person ) ?p2 .
 ?p2 (lp:Person_knows_Person |^lp:Person_knows_Person ) ?p3 .
 ?3 lp:Person_hasInterest_Tag ?tag .
 FILTER ( ?p1 != ?p3 )
}
\end{lstlisting}
